A Detailed Audio-Text Data Simulation Pipeline using Single-Event Sounds

Recently, there has been an increasing focus on audio-text cross-modal learning. However, most of the existing audio-text datasets contain only simple descriptions of sound events. Compared with classification labels, the advantages of such descriptions are significantly limited. In this paper, we first analyze the detailed information that human descriptions of audio may contain beyond sound event labels. Based on the analysis, we propose an automatic pipeline for curating audio-text pairs with rich details. Leveraging the property that sounds can be mixed and concatenated in the time domain, we control details in four aspects: temporal relationship, loudness, speaker identity, and occurrence number, in simulating audio mixtures. Corresponding details are transformed into captions by large language models. Audio-text pairs with rich details in text descriptions are thereby obtained. We validate the effectiveness of our pipeline with a small amount of simulated data, demonstrating that the simulated data enables models to learn detailed audio captioning.

==> rebuttal.tex <==
Reviewer 30D7 has questions about several details:
1) Freesound queries were manually derived based on cluster labels in Section 2.1.
2) Hyper-parameters like thresholds in Sections 3.1 and 4.1, and attribute distribution are empirical values.
3) In the data generation process, we do not add background noise with a certain probability to simulate situations where no discernible source is continuously present in the real dataset.
4) The two datasets generated in Section 4.1 are combined for fine-tuning. The first dataset uses all categories. However, since some categories contain few samples, to allow more data for fine-tuning while avoiding using the same single-event audio sample too many times, we curate the second dataset using only categories with over 200 samples. In this way, over-fitting is partly mitigated as the diversity of single-event audio samples is ensured.

These details will be made clearer in the paper.

Review 387B thinks the comparison is unfair since we involve external data. However, this paper is not about improving the model structure but about proposing a method to generate new audio-text data. The generation process does not require extensive human labeling, so there is no need to ensure the use of consistent training data for comparison.
